Demystifying Swarm Learning: A New Paradigm of Blockchain-based Decentralized Federated Learning

Federated learning (FL) is an emerging promising privacy-preserving machine learning paradigm and has raised more and more attention from researchers and developers. FL keeps users' private data on devices and exchanges the gradients of local models to cooperatively train a shared Deep Learning (DL) model on central custodians. However, the security and fault tolerance of FL have been increasingly discussed, because its central custodian mechanism or star-shaped architecture can be vulnerable to malicious attacks or software failures. To address these problems, Swarm Learning (SL) introduces a permissioned blockchain to securely onboard members and dynamically elect the leader, which allows performing DL in an extremely decentralized manner. Compared with tremendous attention to SL, there are few empirical studies on SL or blockchain-based decentralized FL, which provide comprehensive knowledge of best practices and precautions of deploying SL in real-world scenarios. Therefore, we conduct the first comprehensive study of SL to date, to fill the knowledge gap between SL deployment and developers, as far as we are concerned. In this paper, we conduct various experiments on 3 public datasets of 5 research questions, present interesting findings, quantitatively analyze the reasons behind these findings, and provide developers and researchers with practical suggestions. The findings have evidenced that SL is supposed to be suitable for most application scenarios, no matter whether the dataset is balanced, polluted, or biased over irrelevant features.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> Sections/introduction_1022.tex <==
In benefit of Deep Learning (DL), recent years have witnessed significant progress in multiple tasks in Computer Vision (CV)~\cite{DBLP:conf/nips/KrizhevskySH12} and Natural Language Process (NLP)~\cite{DBLP:journals/nn/GravesS05, DBLP:journals/jmlr/CollobertWBKKK11}. The performance of DL relies on not only appropriate algotithms~\cite{DBLP:journals/nature/LeCunBH15}, but also representative large datasets because it usually leads to overfitting to fit a small dataset into a neural network with numerous parameters. However, in many real-world scenarios, such as medical institutions, Internet of Things (IoT) devices, \textit{etc.}, data are distributed in a decentralized manner. Therefore, the volume of local data is insufficient to train reliable and robust models. It is a common practice to feed local data into a global model and train in a centralized manner to address the local limitations. Undoubtedly, it raises concerns about data ownership, confidentiality, privacy, security, and the creation of data monopolies that favor data aggregators. Recently, the emerging popular Federated Learning (FL)~\cite{DBLP:conf/aistats/McMahanMRHA17} mitigates some of those concerns, where data are kept locally and local confidentiality issues are addressed~\cite{DBLP:conf/ccs/ShokriS15}. Although FL has drawn numerous attention from researchers and developers~\cite{DBLP:conf/www/MaZ00H21, DBLP:conf/www/LiNJZY21, DBLP:conf/www/Liu0C21, DBLP:conf/www/YangWXCBLL21, DBLP:conf/www/ZhangWP21, DBLP:conf/www/Wu0HNWCYZ21}, it uses central custodians to keep model parameters, which could still be attacked to infer users' identities and interests~\cite{DBLP:conf/infocom/WangSZSWQ19, DBLP:conf/sp/NasrSH19, DBLP:journals/jsac/SongWZSWRQ20, DBLP:journals/tifs/ContiMSV16, DBLP:conf/cns/WangYKH15}, even with privacy-preserving deep learning techniques~\cite{DBLP:conf/iotdi/RodriguezWZMH18, goldreich1998secure, DBLP:journals/tifs/ZhaoWZZC20, DBLP:conf/sose/FuWXMW19, DBLP:journals/tifs/DongWWG18, DBLP:conf/atis/PhongA0WM17, DBLP:journals/ejisec/FontaineG07, DBLP:journals/corr/XieBFGLN14}. Besides, the star-shaped architecture of FL damages fault tolerance.

To address the preceding problems raised by FL, Swarm Learning (SL)~\cite{warnat2021swarm} is proposed as a new FL paradigm to combine decentralized hardware infrastructures, distributed machine learning with a permissioned blockchain to securely on-board members, dynamically elect the leader among members, and merge model parameters. %In benefit of the completely decentralized properties of SL, it (1) keeps data locally with the data owner, (2) requires no exchange of raw data, thereby also reducing data traffic, (3) provides high-level data security, (4) guarantees secure, transparent and fair onboarding of decentral members of the network without the need for a central custodian, (5) allows parameter merging with equal rights for all members, and (6) protects machine learning models from attacks~\cite{warnat2021swarm}.
As shown in Figure~\ref{architecture}, SL shares the parameters via the Swarm network and builds the models independently on private data at individual Swarm edge nodes, without the need of a central custodian. In benefit of the private permissioned blockchain, SL secures data sovereignty, security, and confidentiality. Each participant is well defined and only pre-authorized participants can be on-boarded and execute transactions. In the workflow of SL, a new node enrolls via a blockchain smart contract, obtains the model, and performs localized training until a user-defined Synchronization Interval (SI). Then, local model parameters are exchanged and merged to update the global model before the next training round starts. %update the global model via a Swarm application programming interface (API) %In each node, SL contains a middleware layer and an application layer. The middleware layer contains the machine learning platform, the blockchain, and the SL library, which contains encapsulated Swarm APIs to execute SL in heterogeneous hardware infrastructures. The application layer contains the models.
\begin{figure}[htbp]
  \centering
  \vspace{-0.2cm}  %调整图片与上文的垂直距离
  \setlength{\abovecaptionskip}{-0.1cm}   %调整图片标题与图距离
  \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
  \includegraphics[width=0.3\textwidth]{Pictures/SwarmLearning.png}
  \caption{The architecture of Swarm Learning}
  \label{architecture}
  \Description{}
\end{figure}

Despite the increasing attention on the SL paradigm both in industries and in academics, there lacks comprehensive knowledge of best practices and precautions of deploying SL in real-world scenarios. Related work in SL~\cite{lalitha2018fully, DBLP:journals/corr/abs-1901-11173, DBLP:conf/blockchain2/RamananN20, DBLP:journals/corr/abs-2101-06905, DBLP:journals/network/LiCLHZY21, warnat2020swarm, warnat2021swarm} has not made their code available online or only open-sourced the Swarm Learning Library (SLL) in binary format for non-commercial use under evaluation license\footnote{https://github.com/HewlettPackard/swarm-learning}. Although this project has been followed by many researchers and developers, numerous issues about deployment have been raised, such as adaption on different datasets or distributions, encapsulated features, license assignment, connectivity, heterogeneity in operation systems, hardware settings, DL platforms, and models. We use several publicly available datasets and mainstream DL models to address these issues and measure SL in real-world development. Specifically, how does SL perform in terms of prediction accuracy (\textit{RQ1, RQ2, RQ3, RQ4})? How dose SL perform in terms of resource overhead (\textit{RQ1, RQ5})? Besides, considering real-world scenarios make experimental results on standardized datasets invalid, how does SL perform in face of unbalanced datasets (\textit{RQ2}), biased datasets over irrelevant features (\textit{RQ3}), or polluted datasets (\textit{RQ4})? Moreover, whether and how much does scaling the peers in SL affect resource overhead of SL (\textit{RQ5})? 
%\xzl{I still have some concerns about the motivation. You had better try to use some questions, e.g., how the SL performs in terms of prediction accuracy? whether and how much does the imbalance impact the SL? whethter the blockchain impact .....? blablabla...By this you can make readers have more interests to understand why measuring SL matters and fast locate the research questions you raise in the following.}
Besides, we formulate the SL paradigm, quantitatively analyze the possible reasons behind the findings, discuss encapsulated features, and provide developers with practical suggestions on what is recommended, what is not recommended, and where to improve in SL. 
%\xzl{Why is important of lacking the knowledge? Say something here.}
As far as we are concerned, this paper is the first comprehensively empirical study focusing on the SL paradigm. We will make the source code of this paper publicly available online when this paper is accepted. Our findings of this paper can be summarized as follows.
\begin{itemize}
    \item The accuracy of SL is similar to that of Centralized Learning (CL), even if the dataset is unbalanced or polluted.
    %\xzl{Rephrase this para}
    \item When the dataset is biased over irrelevant features, models trained on different SL nodes provide similar accuracy for the same testing set. Therefore, the fairness of SL is better than that of CL.
    %\xzl{What do you mean by ``fairness''}
    \item SL nodes take turns consuming much more compute resources and network resources than other nodes. Besides, some SL nodes consume much more network bandwidth than other SL nodes.
    \item As the number of Swarm Network (SN) nodes increases, resource overhead remains basically unchanged. As the number of SL nodes increases, compute overhead and network overhead increase linearly, while storage overhead remains unchanged.
\end{itemize}

%\xzl{I still have no idea of why making our study of SL matters....}
The remainder of this paper is organized as follows. In Section~\ref{Section:Background}, we introduce the concepts of SL in detail. In Section~\ref{Section:Methodology}, we describe the datasets and models for measuring SL. In Section~\ref{Section:RQs}, we measure the performance, the effect of imbalance, the fairness, fault tolerance, and the scalability of SL. In Section~\ref{Section:Formulation}, we provide quantitative explanation for experimental results. In Section~\ref{Section:Implication}, we provide suggestions for developers and researchers focusing on SL. In Section~\ref{Section:Discussion}, we discuss some limitations of this work and show possible solutions. In Section~\ref{Section:RelatedWork}, we compare this work with related work. Finally, Section~\ref{Section:Conclusion} concludes the paper.
